Cavity-aided magnetic-resonance microscopy of atoms in optical lattices

Magnetic resonance imaging (MRI) is a powerful technique for investigating the microscopic properties and dynamics of physical systems. In this work we demonstrate state-sensitive MRI of ultracold atoms in an optical lattice. Single-shot spatial resolution is 120 nm, well below the lattice spacing, and number sensitivity is +/-2.4 for 150 atoms on a single site, well below Poissonian atom-number fluctuations. We achieve this by combining high-spatial-resolution control over the atomic spin using an atom chip, together with nearly quantum-limited spin measurement, obtained by dispersively coupling the atoms to light in a high-finesse optical cavity. The MRI is minimally disruptive of the atoms' internal state, preserving the magnetisation of the gas for subsequent experiments. Using this technique, we observe the nonequilibrium transport dynamics of the atoms among individual lattice sites. We see the atom cloud initially expand ballistically, followed by the onset of interaction-inhibited transport.

==> mri-v7-main-bib.tex <==
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{bakr09microscope}
\bibinfo{author}{Bakr, W.~S.} \emph{et~al.}
\newblock \bibinfo{title}{A quantum gas microscope for detecting single atoms
  in a {Hubbard-regime} optical lattice}.
\newblock \emph{\bibinfo{journal}{Nature}} \textbf{\bibinfo{volume}{462}},
  \bibinfo{pages}{74--77} (\bibinfo{year}{2009}).

\bibitem{Sherson2010}
\bibinfo{author}{Sherson, J.~F.} \emph{et~al.}
\newblock \bibinfo{title}{Single-atom-resolved fluorescence imaging of an
  atomic {Mott} insulator}.
\newblock \emph{\bibinfo{journal}{Nature}} \textbf{\bibinfo{volume}{467}},
  \bibinfo{pages}{68--72} (\bibinfo{year}{2010}).

\bibitem{schr04register}
\bibinfo{author}{Schrader, D.} \emph{et~al.}
\newblock \bibinfo{title}{Neutral atom quantum register}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{93}}, \bibinfo{pages}{150501}
  (\bibinfo{year}{2004}).

\bibitem{Vengalattore2007:Magnetometry}
\bibinfo{author}{Vengalattore, M.} \emph{et~al.}
\newblock \bibinfo{title}{High-resolution magnetometry with a spinor
  {Bose-Einstein} condensate}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{98}}, \bibinfo{pages}{200801}
  (\bibinfo{year}{2007}).

\bibitem{shin08phasediagram}
\bibinfo{author}{Shin, Y.~I.}, \bibinfo{author}{Schunck, C.~H.},
  \bibinfo{author}{Schirotzek, A.} \& \bibinfo{author}{Ketterle, W.}
\newblock \bibinfo{title}{Phase diagram of a two-component {Fermi} gas with
  resonant interactions}.
\newblock \emph{\bibinfo{journal}{Nature}} \textbf{\bibinfo{volume}{451}},
  \bibinfo{pages}{689--693} (\bibinfo{year}{2008}).

\bibitem{ho10phasediagram}
\bibinfo{author}{Ho, T.~L.} \& \bibinfo{author}{Zhou, Q.}
\newblock \bibinfo{title}{Obtaining the phase diagram and thermodynamic
  quantities of bulk systems from the densities of trapped gases}.
\newblock \emph{\bibinfo{journal}{Nature Physics}}
  \textbf{\bibinfo{volume}{6}}, \bibinfo{pages}{66--69} (\bibinfo{year}{2010}).

\bibitem{navo10eqstate}
\bibinfo{author}{Navon, N.}, \bibinfo{author}{Nascimbene, S.},
  \bibinfo{author}{Chevy, F.} \& \bibinfo{author}{Salomon, C.}
\newblock \bibinfo{title}{The equation of state of a low-temperature {Fermi}  gas with tunable interactions}.
\newblock \emph{\bibinfo{journal}{Science}} \textbf{\bibinfo{volume}{328}},
  \bibinfo{pages}{729--732} (\bibinfo{year}{2010}).

\bibitem{hori10}
\bibinfo{author}{Horikoshi, M.}, \bibinfo{author}{Nakajima, S.},
  \bibinfo{author}{Ueda, M.} \& \bibinfo{author}{Mukaiyama, T.}
\newblock \bibinfo{title}{Measurement of universal thermodynamic functions for
  a unitary {Fermi} gas}.
\newblock \emph{\bibinfo{journal}{Science}} \textbf{\bibinfo{volume}{327}},
  \bibinfo{pages}{442--445} (\bibinfo{year}{2010}).

\bibitem{kuhr:arxiv:addressing}
\bibinfo{author}{Weitenberg, C.} \emph{et~al.}
\newblock \bibinfo{title}{Single-spin addressing in an atomic mott insulator}.
\newblock \bibinfo{note}{arXiv:1101.2076} (\bibinfo{year}{2011}).

\bibitem{ott:prl:addressing}
\bibinfo{author}{W\"urtz, P., Langen, T., Gericke, T., Koglbauer, A., \& Ott, H.}
\bibinfo{title}{Experimental demonstration of single-site addressability in a two-dimensional optical lattice},
\emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}} \textbf{\bibinfo{volume}{103}}, \bibinfo{pages}{080404} (\bibinfo{year}{2009}).

\bibitem{sche00co2lattice}
\bibinfo{author}{Scheunemann, R.}, \bibinfo{author}{Cataliotti, F.~S.},
  \bibinfo{author}{Hansch, T.~W.} \& \bibinfo{author}{Weitz, M.}
\newblock \bibinfo{title}{Resolving and addressing atoms in individual sites of
  a {CO2-laser} optical lattice}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ A}} \textbf{\bibinfo{volume}{62}},
  \bibinfo{pages}{051801} (\bibinfo{year}{2000}).

\bibitem{nels07}
\bibinfo{author}{Nelson, K.~D.}, \bibinfo{author}{Li, X.} \&
  \bibinfo{author}{Weiss, D.~S.}
\newblock \bibinfo{title}{Imaging single atoms in a three-dimensional array}.
\newblock \emph{\bibinfo{journal}{Nature Physics}}
  \textbf{\bibinfo{volume}{3}}, \bibinfo{pages}{556--560}
  (\bibinfo{year}{2007}).

\bibitem{kars09nearest}
\bibinfo{author}{Karski, M.} \emph{et~al.}
\newblock \bibinfo{title}{Nearest-neighbor detection of atoms in a {1D} optical
  lattice by fluorescence imaging}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{102}}, \bibinfo{pages}{053001}
  (\bibinfo{year}{2009}).

\bibitem{geri08ebeam}
\bibinfo{author}{Gericke, T.} \emph{et~al.}
\newblock \bibinfo{title}{High-resolution scanning electron microscopy of an
  ultracold quantum gas}.
\newblock \emph{\bibinfo{journal}{Nature Physics}}
  \textbf{\bibinfo{volume}{4}}, \bibinfo{pages}{949--953}
  (\bibinfo{year}{2008}).

\bibitem{meschede:prl:qjs}
\bibinfo{author}{Khudaverdyan, M.} \emph{et~al.}
\newblock \bibinfo{title}{Quantum jumps and spin dynamics of interacting atoms
  in a strongly coupled atom-cavity system}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{103}}, \bibinfo{pages}{123006}
  (\bibinfo{year}{2009}).

\bibitem{reichel:prl:cavbec}
\bibinfo{author}{Gehr, R.} \emph{et~al.}
\newblock \bibinfo{title}{Cavity-based single atom preparation and
  high-fidelity hyperfine state readout}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{104}}, \bibinfo{pages}{203602}
  (\bibinfo{year}{2010}).

\bibitem{leroux:prl:squeeze}
\bibinfo{author}{Leroux, I.~D.}, \bibinfo{author}{Schleier-Smith, M.~H.} \&
  \bibinfo{author}{Vuleti\ifmmode~\acute{c}\else \'{c}\fi{}, V.}
\newblock \bibinfo{title}{Implementation of cavity squeezing of a collective
  atomic spin}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{104}}, \bibinfo{pages}{073602}
  (\bibinfo{year}{2010}).

\bibitem{meschede:njp:nmr}
\bibinfo{author}{Karski, M.} \emph{et~al.}
\newblock \bibinfo{title}{Imprinting patterns of neutral atoms in an optical
  lattice using magnetic resonance techniques}.
\newblock \emph{\bibinfo{journal}{New J.\ Phys.}} \textbf{\bibinfo{volume}{12}},
  \bibinfo{pages}{065027} (\bibinfo{year}{2010}).

\bibitem{brah10csod}
\bibinfo{author}{Brahms, N.} \& \bibinfo{author}{Stamper-Kurn, D.~M.}
\newblock \bibinfo{title}{Spin optodynamics analog of cavity optomechanics}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ A}} \textbf{\bibinfo{volume}{82}},
  \bibinfo{pages}{041804} (\bibinfo{year}{2010}).

\bibitem{murc08backaction}
\bibinfo{author}{Murch, K.~W.}, \bibinfo{author}{Moore, K.~L.},
  \bibinfo{author}{Gupta, S.} \& \bibinfo{author}{Stamper-Kurn, D.~M.}
\newblock \bibinfo{title}{Observation of quantum-measurement backaction with an
  ultracold atomic gas}.
\newblock \emph{\bibinfo{journal}{Nature Physics}}
  \textbf{\bibinfo{volume}{4}}, \bibinfo{pages}{561--564} (\bibinfo{year}{2008}).

\bibitem{bren08opto}
\bibinfo{author}{Brennecke, F.}, \bibinfo{author}{Ritter, S.},
  \bibinfo{author}{Donner, T.} \& \bibinfo{author}{Esslinger, T.}
\newblock \bibinfo{title}{Cavity optomechanics with a {Bose-Einstein}
  condensate}.
\newblock \emph{\bibinfo{journal}{Science}} \textbf{\bibinfo{volume}{322}},
  \bibinfo{pages}{235--238} (\bibinfo{year}{2008}).

\bibitem{purd10tunable}
\bibinfo{author}{Purdy, T.} \emph{et~al.}
\newblock \bibinfo{title}{Tunable optomechanics with ultracold atoms}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{105}}, \bibinfo{pages}{133701}
  (\bibinfo{year}{2010}).

\bibitem{kuzmich:pra:qnd}
\bibinfo{author}{Kuzmich, A.} \emph{et~al.}
\newblock \bibinfo{title}{Quantum nondemolition measurements of collective
  atomic spin}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ A}} \textbf{\bibinfo{volume}{60}},
  \bibinfo{pages}{2346--2350} (\bibinfo{year}{1999}).

\bibitem{rowland:tomography}
\bibinfo{author}{Rowland, S.~W.}
\newblock \bibinfo{title}{Computer implementation of image reconstruction
  formulas}.
\newblock In \bibinfo{editor}{Herman, G.~T.} (ed.)
  \emph{\bibinfo{booktitle}{Image Reconstruction from Projections}}
  (\bibinfo{publisher}{Springer-Verlag}, \bibinfo{address}{Berlin},
  \bibinfo{year}{1979}), \bibinfo{edition}{1st} edn.

\bibitem{este08squeeze}
\bibinfo{author}{Esteve, J.} \emph{et~al.}
\newblock \bibinfo{title}{Squeezing and entanglement in a {Bose-Einstein}
  condensate}.
\newblock \emph{\bibinfo{journal}{Nature}} \textbf{\bibinfo{volume}{455}},
  \bibinfo{pages}{1216--1219} (\bibinfo{year}{2008}).

\bibitem{oberthaler:prl:selftrap}
\bibinfo{author}{Anker, T.} \emph{et~al.}
\newblock \bibinfo{title}{Nonlinear self-trapping of matter waves in periodic
  potentials}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{94}}, \bibinfo{pages}{020403}
  (\bibinfo{year}{2005}).

\bibitem{Jessen2009:PRL:MicrowaveControl}
\bibinfo{author}{F\"orster, L.} \emph{et~al.}
\newblock \bibinfo{title}{Microwave control of atomic motion in optical
  lattices}.
\newblock \emph{\bibinfo{journal}{Phys.\ Rev.\ Lett.}}
  \textbf{\bibinfo{volume}{103}}, \bibinfo{pages}{233001}
  (\bibinfo{year}{2009}).

\end{thebibliography}

